Exact Computation of a Manifold Metric, via Lipschitz Embeddings and Shortest Paths on a Graph

Data-sensitive metrics adapt distances locally based the density of data points with the goal of aligning distances and some notion of similarity. In this paper, we give the first exact algorithm for computing a data-sensitive metric called the nearest neighbor metric. In fact, we prove the surprising result that a previously published $3$-approximation is an exact algorithm. The nearest neighbor metric can be viewed as a special case of a density-based distance used in machine learning, or it can be seen as an example of a manifold metric. Previous computational research on such metrics despaired of computing exact distances on account of the apparent difficulty of minimizing over all continuous paths between a pair of points. We leverage the exact computation of the nearest neighbor metric to compute sparse spanners and persistent homology. We also explore the behavior of the metric built from point sets drawn from an underlying distribution and consider the more general case of inputs that are finite collections of path-connected compact sets. The main results connect several classical theories such as the conformal change of Riemannian metrics, the theory of positive definite functions of Schoenberg, and screw function theory of Schoenberg and Von Neumann. We develop novel proof techniques based on the combination of screw functions and Lipschitz extensions that may be of independent interest.

==> NN.tex <==
\section{Exactly Computing the nearest neighbor metric}
\label{sec:NN}
In this section, we prove Theorem~\ref{thm:NN} on finite point sets, and
explain in Section~\ref{sec:bodies} that our proof strategy applies to
finite collections of path-connected compact bodies.

  First, lets observe what happens when $P$ has only two points $a$ and
$b$, $\dist_2(a,b) = \dist_N(a,b)$.  This reduces to a high school calculus
exercise as the minimum path $\gamma$ will be a straight line between the
points and the nearest neighbor metric is \[
    \dist_N(a,b) = 4\int_0^1 \distto_P(\gamma(t))\|\gamma'(t)\|dt = 8\int_0^{\frac{1}{2}} t \|a - b\|^2 dt = \|a - b\|^2 = \dist_2(a,b).
  \]
  Now it is easy to observe that the
  nearest neighbor metric is never greater than the
  edge-squared distance, as proven in the following lemma.

  \begin{lemma}\label{lem:dist_N_le_dist}
    For all $s,p\in P$, we have $\dist_N(s,p)\le \dist_2(s,p)$.
  \end{lemma}
  \begin{proof}
    Fix any points $s,p\in P$.
    Let $q_0,\ldots, q_k \in P$ be such that $q_0 = s$, $q_k = p$ and
    \[
      \dist_2(s,p) = \sum_{i=1}^k \|q_i - q_{i-1}\|^2.
    \]
    Let $\psi_i(t) = tq_i + (1-t)q_{i-1}$ be the straight line segment from $q_{i-1}$ to $q_i$.
    Observe that $\len(\psi_i) = \|q_i - q_{i-1}\|^2 / 4$, by the same argument as in the two point case.
    Then, let $\psi$ be the concatenation of the $\psi_i$ and it follows that
    \[
      \dist_2(s,p) = 4 \len(\psi) \ge 4 \inf_{\gamma\in \ourpath(s,p)} \len(\gamma) = \dist_N(s,p).\qedhere
    \]
  \end{proof}
By Lemma~\ref{lem:dist_N_le_dist}, it suffices to show that $\dist_N(a, b) \geq \dist_2(a,b)$ for all $a, b \in P$.
% This allows us to compute of the nearest neighbor metric exactly by instead computing the edge-squared metric.
\input{proof}


==> boxes.tex <==
% !TeX root = main.tex

\subsubsection{Boxes} % (fold)
\label{sec:boxes}

  Let $Q$ be the vertices of a box in $\R^n$.
  That is, there exist some positive real numbers $\alpha_1,\ldots , \alpha_n$ such that each $q\in Q$ can be written as $q = \sum_{i\in I} \alpha_i e_i$, for some $I\subseteq [n]$.

  Let the source $s$ be the origin.
  Let $\distto_Q:\R^n\to \R$ be the distance function to the set $Q$.
  Setting $r_i(x) := \min\{x_i, \alpha_i - x_i\}$ (a lower bound on the difference in the $i$th coordinate to a vertex of the box), it follows that
  \begin{equation}
    \label{eq:distto_bded_by_ris}
    \distto_Q(x) \ge \sqrt{\sum_{i= 1}^n r_i(x)^2}.
  \end{equation}

  Let $\gamma:[0,1]\to \R^n$ be a curve in $\R^n$.
  Define $\gamma_i(t)$ to be the projection of $\gamma$ onto its $i$th coordinate.
  Thus,
  \begin{equation}\label{eq:ri_as_min}
    r_i(\gamma(t)) = \min\{\gamma_i(t), \alpha_i - \gamma_i(t)\}
  \end{equation}
  and
  \begin{equation}\label{eq:gamma_decomposed}
    \|\gamma'(t)\| = \sqrt{\sum_{i = 1}^n \gamma_i'(t)^2}.
  \end{equation}
  %
  We can bound the length of $\gamma$ as follows. For simplicity of exposition we only present the case
  of a path from the origin to the far corner, $p = \sum_{i=1}^n \alpha_i e_i$. 
  %
  \begin{align*}
    \len(\gamma)
      &= \int_0^1 \distto_Q(\gamma(t))\|\gamma'(t)\|dt \because{by definition}\\
      &\ge \int_0^1 \left(\sqrt{\sum_{i= 1}^n r_i(\gamma(t))^2} \sqrt{\sum_{i = 1}^n \gamma_i'(t)^2}\right) dt \because{by \eqref{eq:distto_bded_by_ris} and \eqref{eq:gamma_decomposed}}\\
      &\ge \sum_{i=1}^n \int_0^1 r_i(\gamma(t)) \gamma_i'(t) dt \because{Cauchy-Schwarz}\\
      &\ge \sum_{i=1}^n \left(\int_0^{\ell_i} \gamma_i(t) \gamma_i'(t)dt + \int_{\ell_i'}^1 (\alpha_i - \gamma_i(t)) \gamma_i'(t) dt\right) \\ \because{by \eqref{eq:ri_as_min} where $\gamma_i(\ell_i) = \alpha_i/2$ for the first time and $\gamma_i(\ell_i') = \alpha_i/2$ for the last time.}\\
      &= \sum_{i=1}^n 2\int_0^{\ell_i} \gamma_i(t) \gamma_i'(t) dt \because{by symmetry}\\
      &\ge \sum_{i=1}^n \frac{\alpha_i^2}{4} \because{basic calculus}
  \end{align*}

  It follows that if $\gamma$ is any curve that starts at $s$ and ends at $p = \sum_{i=1}^n \alpha_i e_i$, then $\dist_N(s,p) = \dist_2(s,p)$.

% section boxes (end)


==> environments.tex <==
\newtheorem{claim}{Claim}
\newtheorem{observation}{Observation}
\newtheorem{problem}{Problem}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{remark}{Remark}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}


==> lifting.tex <==
\subsubsection{Lifting the points to $\R^n$} % (fold)
\label{sec:lifting}

  Define a mapping $m: P \to \R^n$.  We do this by adding the points $p_1, \ldots, p_n$, as defined above, one point at a time.
  For each new point we will introduce a new dimension. We start by setting $m(p_1) = 0$ and by induction:
  \begin{equation}\label{eq:defn_of_m}
    m(p_i) = m(p_{i-1}) + \sqrt{\dist_2(s, p_i) - \dist_2(s, p_{i-1})} e_i,
  \end{equation}
  where the vectors $e_i$ are the standard basis vectors in $\R^n$.
  A similar embedding works for some other functions and was extensively studied by Schoenberg and Von Neumann in the theory of screw functions.

  \begin{lemma}\label{lem:m_and_dist}
    For all $p_i, p_j\in P$, we have
    \begin{enumerate}
      \item[(i)] $\|m(p_j) - m(p_i)\| = \sqrt{|\dist_2(s,p_j) - \dist_2(s,p_i)|}$, and
      \item[(ii)]$\|m(s) - m(p_j)\|^2 \le \|m(p_i)\|^2 + \|m(p_i) - m(p_j)\|^2$.
    \end{enumerate}
  \end{lemma}
  \begin{proof}
    \emph{Proof of (i).}
    Without loss of generality, let $i \le j$.
    \begin{align*}
      \|m(p_j) - m(p_i)\| &= \left\|\sum_{k=i+1}^j \sqrt{\dist_2(s, p_k) - \dist_2(s, p_{k-1})} e_k \right\| \because{from the definition of $m$}\\
      &= \sqrt{\sum_{k=i+1}^j (\dist_2(s, p_k) - \dist_2(s, p_{k-1}))}\because{expand the norm}\\
      &= \sqrt{\dist_2(s, p_j) - \dist_2(s, p_i)}. \because{telescope the sum}
    \end{align*}

    \noindent\emph{Proof of (ii).}
    As $m(s) = 0$, it suffice to observe that
    \begin{align*}
      \|m(p_j)\|^2
        &= \dist_2(s, p_j) \because{by \emph{(i)}}\\
        &\le \dist_2(s, p_i) + |\dist_2(s,p_j) - \dist_2(s,p_i)|\because{basic arithmetic}\\
        &= \|m_(p_i)\|^2 + \|m(p_i) - m(p_j)\|^2 \because{by \emph{(i)}}
    \end{align*}
  \end{proof}

  We can now show that $m$ has all of the desired properties.

  \begin{prop}\label{prop:m_is_good}
    Let $P\subset\R^d$ be a set of $n$ points, let $s\in P$ be a designated source point, and let $m:P\to \R^n$ be the map defined as in \eqref{eq:defn_of_m}.
    Let $\dist'$ denote the edge squared metric for the point set $m(P)$ in $\R^n$.
    Then,
    \begin{enumerate}
      \item[(i)] $m$ is $1$-Lipschitz as a map between Euclidean metrics,
      \item[(ii)] $m$ maps the points of $P$ to the vertices of a box, and
      \item[(iii)] $m$ preserves the edge squared distance to $s$, i.e.\ $\dist'(m(s), m(p)) = \dist_2(s,p)$ for all $p\in P$.
    \end{enumerate}
  \end{prop}
  \begin{proof}
    \emph{Proof of (i).} To prove the Lipschitz condition, fix any $a,b\in P$ and bound the distance as follows.
    \begin{align*}
      \|m(a) - m(b)\|
        &= \sqrt{|\dist_2(s,a) - \dist_2(s,b)|} \because{Lemma~\ref{lem:m_and_dist}(i)}\\
        &\le \sqrt{\dist_2(a,b)} \because{triangle inequality}\\
        &\le \|a-b\| \because{$\dist_2(a,b)\le \|a-b\|^2$ by the definition of $\dist$}
    \end{align*}

    \noindent
    \emph{Proof of (ii).} That $m$ maps $P$ to the vertices of a box is immediate from the definition.
    The box has side lengths $\|m_i - m_{i-1}\|$ for all $i>1$ and $p_i = \sum_{k=1}^i \|m_k - m_{k-1}\| e_k$.

    \noindent
    \emph{Proof of (iii).} We can now show that the edge squared distance to $s$ is preserved.
    Let $q_0,\ldots, q_k$ be the shortest sequence of points of $m(P)$ that realizes the edge-squared distance from $m(s)$ to $m(p)$, i.e., $q_0 = m(s)$, $q_k = m(p)$, and
    \[
      \dist'(m(s), m(p)) = \sum_{i = 1}^k \|m(q_i) - m(q_{i-1})\|^2.
    \]
    If $k> 1$, then Lemma~\ref{lem:m_and_dist}(ii) implies that removing $q_1$ gives a shorter sequence.
    Thus, we may assume $k = 1$ and therefore, by Lemma~\ref{lem:m_and_dist}(i),
    \[
      \dist'(m(s), m(p)) = \|m(s) - m(p)\|^2 = \dist_2(s,p).\qedhere
    \]
  \end{proof}


% section lifting (end)


==> lip_extension.tex <==
\subsubsection{The Lipschitz Extension} % (fold)
\label{sec:lip_extension}

  Proposition~\ref{prop:m_is_good} and the Kirszbraun theorem on Lipschitz extensions imply that we can extend $m$ to a $1$-Lipschitz function $f: \R^d\to \R^n$ such that $f(p) = m(p)$ for all $p\in P$ \cite{Kirszbraun1934,Valentine1945,brehm1981}.

  \begin{lemma}\label{lem:dist_N_lipschitz}
    The function $f$ is also $1$-Lipschitz as mapping from $\R^d\to \R^n$ with both spaces endowed with the nearest neighbor metric.
  \end{lemma}
  \begin{proof}
    We are interested in two distance functions $\distto_P:\R^d \to \R$ and $\distto_{f(P)}: \R^n\to \R$.
    Recall that each is the distance to the nearest point in $P$ or $f(P)$ respectively.
    \begin{align*}
      \distto_{f(P)}(f(x)) 
        &= \min_{q\in f(P)} \|q - f(x)\| \because{by definition}\\
        &= \min_{p\in P} \|f(p) - f(x)\| \because{$q = f(p)$ for some $p$}\\
        &\le \min_{p\in P} \|p - x\| \because{$f$ is $1$-Lipschitz}\\ 
        &= \distto_P(x). \because{by definition}
    \end{align*}
    For any curve $\gamma:[0,1]\to \R^d$ and for all $t\in [0,1]$, we have $\|(f\circ \gamma)'(t)\| \le \|\gamma'(t)\|$.
    It then follows that
    \begin{equation}\label{eq:curves_shorten}
      \len'(f\circ \gamma) = \int_0^1 \distto_{f(P)}(f(\gamma(t)))\|(f\circ\gamma)'(t)\|dt \le \int_0^1 \distto_{P}(\gamma(t))\|\gamma'(t)\|dt = \len(\gamma),
    \end{equation}
    where $\len'$ denotes the length with respect to $\distto_{f(P)}$.
    Thus, for all $a,b\in P$,
    \begin{align*}
      \dist_N(a,b)
        &= 4 \inf_{\gamma\in \ourpath(a,b)} \len(\gamma) \because{by definition}\\
        &\ge 4 \inf_{\gamma\in \ourpath(a,b)} \len'(f\circ\gamma) \because{by \eqref{eq:curves_shorten}}\\
        &\ge 4 \inf_{\gamma'\in \ourpath(f(a),f(b))} \len'(\gamma') \because{because $f\circ\gamma\in \ourpath(f(a), f(b))$}\\
        &= \dist_N(f(a), f(b)). \because{by definition}
    \end{align*}
  \end{proof}
  
  We now restate Theorem~\ref{thm:NN} for convenience, and prove
  it.
  \begin{theorem}\label{thm:equality}
    For any point set $P\subset\R^d$, the edge squared metric $\dist$ and the nearest neighbor metric $\dist_N$ are identical.
  \end{theorem}
  \begin{proof}
    Fix any pair of points $s$ and $p$ in $P$.
    Define the Lipschitz mapping $m$ and its extension $f$ as in \eqref{eq:defn_of_m}.
    Let $\dist'$ and $\dist_N'$ denote the edge-squared and nearest neighbor metrics on $f(P)$ in $\R^n$.
    \begin{align*}
      \dist_2(s,p) 
        &= \dist'(m(s), m(p)) \because{Proposition~\ref{prop:m_is_good}(iii)}\\
        &= \dist_N'(m(s), m(p)) \because{$f(P)$ are vertices of a box}\\
        &\le \dist_N(s, p) \because{Lemma~\ref{lem:dist_N_lipschitz}}
    \end{align*}
    We have just shown that $\dist\le \dist_N$ and Lemma~\ref{lem:dist_N_le_dist} states that $\dist\ge \dist_N$, so we conclude that $\dist = \dist_N$ as desired.
  \end{proof}

% section lip_extension (end)


==> old-definitions.tex <==
% !TeX root = main.tex

\section{Definitions} % (fold)
\label{sec:definitions}

\subsection{Definitions for Theorem~\ref{thm:NN}}
  For $x\in \R^d$, let $\|x\|$ denote the Euclidean norm.
  For a set of points $P\subset \R^d$, we can consider some other metrics as well.
  
  
  \begin{definition}
  The \textbf{edge-squared metric} for $a,b\in P$ is
  \[
    \dist_2(a,b) = \min_{(p_0,\ldots, p_k)}\sum_{i=1}^k \|p_i - p_{i-1}\|^2,
  \]
  where the minimum is over sequences of points $p_0,\ldots, p_k\in P$ with $p_0 = a$ and $p_k = b$.
  \end{definition}

  Another metric on the points of $P$ is called the \textbf{nearest neighbor Geodesic} and is denoted $\dist_N$.
  Before we can define it, we need a couple other definitions.

  Given any finite set $P\subset \R^k$, there is a real-valued function $\distto_P: \R^k\to \R$ defined as $\distto_P(z) = \min_{x\in P} \|x-z\|$.
  A path is a continuous mapping $\gamma:[0,1]\to \R^d$.
  Let $\ourpath(a,b)$ denote the set of piecewise-$C_1$ paths from $a$ to $b$.
  We will compute the lengths of paths relative to the distance function $\distto_P$ as follows.
  \[
    \len(\gamma) := \int_0^1 \distto_P(\gamma(t))\|\gamma'(t)\|dt.
  \]
  By considering the velocity of $\gamma$, this definition is
  independent of the parameterization of the path.
  \begin{definition}
    The \textbf{nearest neighbor Geodesic} is defined as:
  \[
    \dist_N(a,b) := 4 \inf_{\gamma\in \ourpath(a,b)}\len(\gamma).
  \]
  The factor of $4$ normalizes the metrics.
  \end{definition}
  In particular, when $P$ has only two points $a$ and $b$, $\dist_2(a,b) = \dist_N(a,b)$.
  This reduces to a high school calculus exercise as the minimum path $\gamma$ will be a straight line between the points and the nearest neighbor distance is
  \[
    \dist_N(a,b) = 4\int_0^1 \distto_P(\gamma(t))\|\gamma'(t)\|dt = 8\int_0^{\frac{1}{2}} t \|a - b\|^2 dt = \|a - b\|^2 = \dist_2(a,b).
  \]

  This observation about pairs of points makes it easy to see that the nearest neighbor distance is never greater than the edge-squared distance as proven in the following lemma.

  \begin{lemma}\label{lem:dist_N_le_dist}
    For all $s,p\in P$, we have $\dist_N(s,p)\le \dist_2(s,p)$.
  \end{lemma}
  \begin{proof}
    Fix any points $s,p\in P$.
    Let $q_0,\ldots, q_k \in P$ be such that $q_0 = s$, $q_k = p$ and
    \[
      \dist_2(s,p) = \sum_{i=1}^k \|q_i - q_{i-1}\|^2.
    \]
    Let $\psi_i(t) = tq_i + (1-t)q_{i-1}$ be the straight line segment from $q_{i-1}$ to $q_i$.
    Observe that $\len(\psi_i) = \|q_i - q_{i-1}\|^2 / 4$, by the same argument as in the two point case.
    Then, let $\psi$ be the concatenation of the $\psi_i$ and it follows that
    \[
      \dist_2(s,p) = 4 \len(\psi) \ge 4 \inf_{\gamma\in \ourpath(s,p)} \len(\gamma) = \dist_N(s,p).\qedhere
    \]
  \end{proof}
  
% section definitions (end)


==> old-introduction.tex <==
\section{Introduction}

A foundational hypothesis in non-linear dimension reduction and machine
learning is that data can be represented as points in Euclidean space,
and that graphs on these points can be generated to solve a variety of
problems on the data, including classification, regression, and clustering \cite{Daitch09, Chen11,vL09, Dong11, Hashi15,
vonluxburg13density, mcqueen16megaman}.
Such graphs can induce similarity measures or distances on the point set,
which are used as the key model when generating a clustering or
classification~\cite{Daitch09, bijral11semiSupLearningDBD, tenenbaum00global}

The problem of generating meaningful graphs and metrics on data is an active research topic in machine learning, statistics, and
geometry~\cite{hein07graph, amenta99surface, sajama05estimatingDBDM, vincent03,
bijral11semiSupLearningDBD, Hashi15, alamgir12shortest, ting10analysis,
gorban07principal, bookDey2007, cavanna16adaptive, Gottlieb14, vL04,
agarwal16efficient, SridharMaster, hwang2016}.
% We believe two important problems are: comparing the
% various methods of generating distances from point sets, and
% building data structures to quickly compute these distances.
%
In this paper, we study a distance generated from a graph
on points in Euclidean space called the edge-squared metric. It
is defined by taking the squared Euclidean distance between every pair of
points, and finding the shortest path on the resulting graph.
This metric has the property that two points
in a dense cluster can be close, even if their Euclidean
distance is far~\cite{bijral11semiSupLearningDBD}.
This property is known as \textbf{density-sensitivity}
~\cite{vincent03}, and is
desirable for clustering and classification
~\cite{sajama05estimatingDBDM, alamgir12shortest, hwang2016,
cohen15approximating}. The edge-squared metric has been studied
before in the
context of machine learning~\cite{bijral11semiSupLearningDBD, vincent03, hwang2016, alamgir12shortest,
cohen15approximating} and
power-efficient wireless
networks~\cite{LiWan2001, LiWan2002}.
Squared Euclidean distances have been
examined before as an optimization objective, and occur in
natural settings including $k$-means clustering and RMS
matching~\cite{macqueen67,Agarwal12}.
We compare the edge-squared metric to another
distance on point sets known as the nearest neighbor metric,
first introduced in~\cite{cohen15approximating} as the nearest neighbor
distance. Close variants of this metric have been studied in
probability and machine learning~\cite{sajama05estimatingDBDM, cohen15approximating,
hwang2016}. We then give efficient algorithms constructing sparse
spanners for both metrics.

% Close variants of both these metrics have been studied in machine
% learning~\cite{bijral11semiSupLearningDBD, LiWan2001,
% alamgir12shortest,sajama05estimatingDBDM, cohen15approximating,
% vincent03, hwang2016}.

In this paper, we show that the edge-squared metric and nearest-neighbor
geodesic distance are
identical. It was not previously known or
suspected that the two might be the same. This is the
first work we know of that equates a discrete metric with a
continuous geodesic, and gives the first nontrivial example of a
so-called \textbf{density-based distance}~\cite{sajama05estimatingDBDM} that can
be computed exactly. This considerably improves a result
in~\cite{cohen15approximating}, which showed that the two were
$3$-approximations of each other. Previous works computing
geodesics or density-based distances generally use approximate
methods whose running time grows as the approximation
quality improves~\cite{Kimmel98, tenenbaum00global,
alamgir12shortest, agarwal16efficient, hwang2016,
cohen15approximating}, or
calculus of variations~\cite{bernoulli, Schwarzschild, Sussmann97}.
We don't follow any of the previous existing approaches. Our proof employs
the Kirszbraun theorem, also known as the Lipschitz
Extension Theorem~\cite{Kirszbraun1934, brehm1981}. This theorem has been
widely used in mathematics, classification, and metric
embeddings~\cite{Naor06, Lee05, Naor15, Gottlieb14, Gottlieb17}.
Our result lets us compute the persistent
homology of the nearest neighbor metric, a general problem of interest for
many continuous metrics in the computational geometry
setting~\cite{edelsbrunner02topological,gasparovic17complete,chazal08towards,chazal13persistence,carlsson09topology}.

In order to perform clustering or classification with the edge-squared
metric or nearest neighbor metric, we
provide data structures that admit fast, practical
computation of these metrics with theoretical guarantees. The
edge-squared metric can have high doubling
dimension even if the underlying points are in $2$
dimensions~\cite{cohen15approximating}. This
means that many data structures suitable for low-doubling dimension
metrics will not immediately
work on it. Despite this, if the underlying point set is in low dimension,
we compute a sparse $(1+\eps)$-spanner of
the edge-squared metric quickly.
This spanner is sparser and faster to compute than the
best known $(1+\eps)$-spanners for Euclidean metrics, and uses
techniques from well-separated pair
decompositions~\cite{Callahan1993} and
approximate Euclidean MSTs~\cite{arya95euclid, Arya2016,
Callahan1995}.

 A foundational assumption of
machine learning is that most data points are samples from a
well-behaved probability
distribution with low intrinsic dimension~\cite{tenenbaum00global,
gorban07principal, vandermaaten08visualizing, Hashi15, mcqueen16megaman,
hwang2016}.
We compute a sparse
$1$-spanner for our metrics in such a setting. Our $1$-spanner is a $k$-nearest neighbor graph ($k$-NN graph)
with edge weights equal to Euclidean distance squared, with $k = O(2^d \log n)$. Here, $d$ is the
intrinsic dimension of the probability density.
Note that a sparse $1$-spanner of
Euclidean distance is not possible in this setting.
Our result may allow for fast computation of edge-squared spanners in
practice, given the breadth of
literature on the $k$-NN graph~\cite{Brito97, Dong11, Chen11}
and its widespread
use in practice~\cite{tenenbaum00global, vL09, Dong11}.
If intrinsic dimension $d$ is constant,
our $k$ is nearly optimal:
it is believed $k=\Omega(\log n)$ is necessary for
connectivity of the $k$-nearest neighbor
graph~\cite{Balister05,Gonzales2003, vL09}.

We also show how spanners of the edge-squared metric can be seen as a generalization of
Euclidean spanners~\cite{Vaidya1991, Elkin2013, arya95euclid,
Callahan1993}, approximate Euclidean
MSTs~\cite{Callahan1995, Andoni2014, Arya2016, Alman2016, Yaro2017}, and
single linkage clustering~\cite{Gower1969, Yaro2017}.\input{definitions}
% To illustrate one finding, we prove in this section that:
% \begin{lemma} \label{lem:one-span} A $1$-spanner of the edge-squared metric
%   contains every Euclidean MST.
% \end{lemma}
% This leads us to an alternate proof of the following corollary, which was already known in the
% literature~\cite{Gonzales2003}:
% \begin{corollary} For a Lipschitz distribution of bounded support bounded
%   above and below, with constant intrinsic
%   dimension $d$, the $k$-NN graph from
%   points drawn from this distribution contains all Euclidean MSTs w.h.p
%   when $k = O(\log n)$. The Euclidean MST is unique almost always.
% \end{corollary}
% \begin{proof} This follows from Theorem~\ref{thm:distribution-spanner}
%   and Lemma~\ref{lem:one-span}.
% \end{proof}
%%%%%% Two techniques!!!

%% In this
%% paper, we provide two techniques for computing accurate and sparse
%% spanners of the edge-squared metric (thus also computing it for the
%% nearest neighbor metric), when the point set lives in constant dimensional space.

%%%%% Two techniques continued!!!!
%% One technique
%% is useful in the setting where the point-set comes from an underlying
%% probability
%% distribution, an assumption common in the machine learning setting. This
%% uses $k$-NN graphs, a common tool in machine learning. The
%% second technique can be used for any point set, and uses well-separated
%% pair decompositions, and other techniques used in computing fast
%% Euclidean spanning trees.

%%%%%%%% Below: Some exposition on the edge^2 metric and NN metric, and what they
%% are.

%% The edge-squared metric is a metric built by taking the graph of
%% Euclidean distances between points, squaring them, and taking the
%% shortest path on the resulting graph. The
%% nearest neighbor metric is a distance based on geodesics through the
%% ambient space, and will be fully
%% defined in Section~\ref{sec:definitions}.


==> persistence.tex <==
\section{Persistent Homology of the Nearest-neighbor Geodesic Distance}
  \label{sec:persistence}

% \tim{This section should be prefaced somewhere -- here or in a previous
% section -- with a statement as to why the nearest neighbor metric may
% still be of independent interest. My main claim is that it's useful
% since it's defined on all points rather than just two.}
%
% \tim{My main issue with this section is that I don't have a clean
% theorem saying how to compute persistent homology, both in ambient and
% intrinsic setting. Having one or two top-level theorems that say this
% would be great, rather than having it be written in the exposition. As
% it stands, I have no clue how Lemma 4.5 is used, or Lemma 4.6, to
% compute the homologies.}
  In this section, we show how to compute the so-called persistent homology~\cite{edelsbrunner02topological} of the nearest neighbor metric in two different ways, one ambient and the other intrinsic.
  The latter relies on Theorem~\ref{thm:NN} and would be quite surprising without it.

  The input for persistence computation is a \emph{filtration}---a nested sequence of spaces, usually parameterized by a real number $\alpha\ge 0$.
  The output is a set of points in the plane called a \emph{persistence diagram} that encodes the birth and death of topological features like connected components, holes, and voids.

  \paragraph*{The Ambient Persistent Homology}

    Perhaps the most popular filtration to consider on a Euclidean space is the sublevel set filtration of the distance to a sample $P$.
    This filtration is $(F_\alpha)_{\alpha\ge 0}$, where
    \[
      F_\alpha := \{x\in \R^d \mid \distto_P(x) \le \alpha\},
    \]
    for all $\alpha \ge 0$.
    If one wanted to consider instead the nearest neighbor metric $\dist_N$, one gets instead a filtration $(G_\alpha)_{\alpha\ge 0}$, where
    \[
      G_\alpha := \{x\in \R^d \mid \min_{p_\in P} \dist_N(x,p) \le \alpha\},
    \]
    for all $\alpha \ge 0$.

    Both the filtrations $(F_\alpha)$ and $(G_\alpha)$ are unions of metric balls.
    In the former, they are Euclidean.
    In the latter, they are the metric balls of $\dist_N$.
    These balls can look very different, for example, for $\dist_N$, the metric balls are likely not even convex.
    However, these filtrations are very closely related.
    \begin{lemma}
      For all $\alpha \ge 0$, $F_\alpha = G_{2\alpha^2}$.
    \end{lemma}
    \begin{proof}
      The key to this exercise is to observe that the nearest point $p \in P$ to a point $x$ is also the point that minimizes $\dist_N(x,p)$.
      To prove this, we will show that for any $p\in P$ and any path $\gamma\in \ourpath(x,p)$, we have $\len(\gamma)\ge \frac{1}{2}\distto_P(x)^2$.
      Consider any such $x$, $p$, and $\gamma$.
      The euclidean length of $\gamma$ must be at least $\distto_P(x)$, so we will assume that $\|\gamma'\| = \distto_P(x)$ and will prove the lower bound on the subpath starting at $x$ of length exactly $\distto_P(x)$.
      This will imply a lower bound on the whole path.
      Because $\distto_P$ is $1$-Lipschitz, we have $\distto_P(\gamma(t))\ge (1-t)\distto_P(x)$ for all $t\in [0,1]$.  It follows that
      \[
        \len(\gamma) = \int_0^1 \distto_P(\gamma(t))\|\gamma'(t)\|dt
          \ge \distto_P(x)^2 \int_0^1 (1-t)dt
          =  \frac{1}{2}\distto_P(x)^2
      \]
      The bound above applies to any path from $x$ to a point $p\in P$, and so,
      \[
        \dist_N(x,p) = 4 \inf_{\gamma\in \ourpath(x,p) \len(\gamma)} \ge 2\distto_P(x).
      \]
      If $p$ is the nearest neighbor of $x$ in $P$, then $\dist_N(x,p) = 2\distto_P(x)$, by taking the path to be a straight line.
      It follows that $\min_{p\in P}\dist_N(x,p) = 2\distto_P(x)$.
    \end{proof}

    The preceding lemma shows that the two filtrations are equal up to a monotone change in parameters.
    By standard results in persistent homology, this means that their persistence diagrams are also equal up to the same change in parameters.
    This means that one could use standard techniques such as $\alpha$-complexes~\cite{edelsbrunner02topological} to compute the persistence diagram of the Euclidean distance and convert it to the nearest neighbor metric afterwards.
    Moreover, one observes that the same equivalence will hold for variants of the nearest neighbor metric that take other powers of the distance.

    % (some are considered in Section~\ref{sec:higher_powers}).


  \paragraph*{Intrinsic Persistent Homology}
    Recently, several researchers have considered intrinsic nerve complexes on metric data, especially data coming from metric graphs~\cite{adamszek16nerve,gasparovic17complete}.
    These complexes are defined in terms of the intersections of metric balls in the input.
    The vertex set is the input point set.
    The edges at scale $\alpha$ are pairs of points whose $\alpha$-radius balls intersect.
    In the intrinsic \v Cech complex, triangles are defined for three way intersections, tetrahedra for four-way intersections, etc.

    In Euclidean settings, little attention was given to the difference between the intrinsic and the ambient persistence, because a classic result, the Nerve Theorem~\cite{borsuk48imbedding}, and its persistent version~\cite{chazal08towards} guaranteed there is no difference.
    The Nerve theorem, however, requires the common intersections to be contractible, a property easily satisfied by convex sets such as Euclidean balls.
    However, in many other topological metric spaces, the metric
    balls might not be so well-behaved.
    In particular, the nearest neighbor metric has metric balls which may take on very strange shapes, depending on the density of the sample.
    This is similarly true for graph metrics.
    So, in these cases, there is a difference between the information in the ambient and the intrinsic persistent homology.

    \begin{theorem}
      Let $P\subset \R^d$ be finite and let $\dist_N$ be the nearest neighbor metric with respect to $P$.
      The edges of the intrinsic \v Cech filtration with respect to $\dist_N$ can be computed exactly in polynomial time.
    \end{theorem}
    \begin{proof}
      The statement is equivalent to the claim that $\dist_N$ can be computed exactly between pairs of points of $P$, a corollary of Theorem~\ref{thm:equality}.
      Two radius $\alpha$ balls will intersect if and only of the distance between their centers is at most $2\alpha$.
      The bound on the distance necessarily implies a path and the common intersection will be the midpoint of the path.
    \end{proof}


==> proof.tex <==
%\subsection{Equivalence} % (fold)
\label{sec:the_proof}

  Let $P\subset \R^d$ be a set of $n$ points.
  Pick any \emph{source} point $s\in P$.
  Order the points of $P$ as $p_1,\ldots ,p_n$ so that
  \[
    \dist_2(s,p_1) \le \cdots \le \dist_2(s, p_n).
  \]
  This will imply that $p_1 = s$.
  It will suffice to show that for all $p_i\in P$, we have $\dist_2(s,p_i) = \dist_N(s,p_i)$.
  There are three main steps:
  \begin{enumerate}
    \item We first show that when $P$ is a subset of the vertices of an axis-aligned box, $\dist = \dist_N$.  In this case, shortest paths for $\dist$ are single edges and shortest paths for $\dist_N$ are straight lines.
    \item We then show how to lift the points from $\R^d$ to $\R^n$ by a Lipschitz map $m$ that places all the points on the vertices of a box and preserves $\dist_2(s,p)$ for all $p\in P$.
    \item Finally, we show how the Lipschitz extension of $m$ is also Lipschitz as a function between nearest neighbor metrics.  We combine these pieces to show that $\dist \le \dist_N$.  As $\dist \ge \dist_N$ (Lemma~\ref{lem:dist_N_le_dist}), this will conclude the proof that $\dist = \dist_N$.
  \end{enumerate}
The key to the second step, to be elaborated in Section~\ref{sec:lifting},
is that if you take points on a line and raise the pairwise distances to
the $1/2$ power, you get points on a box. This is a special case of the
general theory on screw functions developed by Von Neumann and Schoenberg,
which asserts a far more general criterion on when functions applied to
pairwise distances between points on a line can be embedded into Euclidean
space~\cite{VonNeumann41}.
  \input{boxes}
  \input{lifting}
  \input{lip_extension}
\subsection{From Finite Sets to Finite Collections of Compact Path-Connected Bodies}
\label{sec:bodies}
All of our proof steps hold for finite collections of compact,
path-connected bodies in arbitrarily large dimension. Our Lipschitz map $m$ can
still be extended to a Lipschitz map $f$ in this setting, largely due to the
generality of the Kirszbraun theorem. In this case, the pre-image of the
contractive map is the set of all points belonging to some body. Meanwhile, the image is a finite set of points, the corners of a multi-dimensional box.
Thus our construction of $m$ contracts each convex
body into a single point, and the image of our
compact bodies under $f$ is still a finite point set on the corners of a
box. Therefore, the remainder of our theorem proof goes through unchanged.

This result is rather remarkable: path-connected compact sets in high
dimensional space can have extremely convoluted geometry, and the Voronoi diagrams
on these collections (on which the nearest neighbor metric depends) can be
massively complex.  The key is that our Lipschitz map is robust enough to
handle objects of considerable geometric complexity.
  
  
% section the_proof (end)


==> relation-to-MST.tex <==
\section{Relation to MST distances, and other distances in Geometry}


==> spanner.tex <==
\section{Spanners for the nearest neighbor metric}
In this section, we prove our theorems on spanners of the nearest neighbor
metric. The proofs of these theorems mostly leverage Theorem~\ref{thm:NN}
and past work on geometric spanners. We have nonetheless included them
for completeness, and to illustrate that spanners of
manifold distances like the nearest neighbor metric can have interesting
properties not found in Euclidean spanners (assuming no Steiner points).
\input{distribution-spanner}
\input{general-spanner}

